DrVideo: Document Retrieval Based Long Video Understanding

Most of the existing methods for video understanding primarily focus on videos only lasting tens of seconds, with limited exploration of techniques for handling long videos. The increased number of frames in long videos poses two main challenges: difficulty in locating key information and performing long-range reasoning. Thus, we propose DrVideo, a document-retrieval-based system designed for long video understanding. Our key idea is to convert the long-video understanding problem into a long-document understanding task so as to effectively leverage the power of large language models. Specifically, DrVideo first transforms a long video into a coarse text-based long document to initially retrieve key frames and then updates the documents with the augmented key frame information. It then employs an agent-based iterative loop to continuously search for missing information and augment the document until sufficient question-related information is gathered for making the final predictions in a chain-of-thought manner. Extensive experiments on long video benchmarks confirm the effectiveness of our method. DrVideo significantly outperforms existing LLM-based state-of-the-art methods on EgoSchema benchmark (3 minutes), MovieChat-1K benchmark (10 minutes), and the long split of Video-MME benchmark (average of 44 minutes).

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/sections/intro.tex <==
\section{Introduction}

%The recent success of large-scale pre-trained language models\cite{brown2020language,chung2024scaling,touvron2023llama} has led to a burst of multimodal vision-and-language models that can jointly understand visual (image/video) and language data\cite{cho2021unifying,sun2019videobert}. However, due to higher computational and annotation costs, video-language models (video-LMs) are more challenging to scale in terms of model and data size than image-language models (image-LMs). \chenhui{Change here} Hence, recent studies have explored efficient training of video-LMs by leveraging pre-trained image-LMs\cite{ju2022prompting,yang2022zero,lei2021less,maaz2023video,zhang2023video,yu2024self}. These works try to select subsets of frames, either through uniform sampling or keyframe selection. Despite promising performance achieved by these works, they mainly focus on video of ten of seconds.\par
Video understanding is a challenging task in computer vision, requiring the processing of spatio-temporal information and advanced reasoning abilities. Previous works have successfully processed short videos lasting around tens of seconds~\cite{yang2021just, VindLU_CVPR2023, lei2021less, yu2023self, yang2022zero, suris2023vipergpt, lin2023mm}. However, how to extend these methods to long videos remains unclear. Recent advancements in large language models (LLMs) ~\cite{instructGPT, chatgpt, gpt3, bloom, llama, chowdhery2022palm, ma2024gerea} demonstrate strong abilities in language understanding and reasoning across long text sequences. These advancements have inspired the development of video-language models (Video-LMs) to address long video understanding issues. 
\begin{figure}[t]
    \centering
    %\includegraphics[width=90mm]{latex/image/drvideo_1.pdf}
    \includegraphics[width=\linewidth]{./image/drvideo_1.pdf}
    %\end{adjustbox}
\caption{\textbf{Accuracy on EgoSchema \cite{mangalam2023egoschema}, MovieChat-1K\cite{song2023moviechat} global mode, and LLama-Vid-QA \cite{LLaMA-VID}}. Our method, DrVideo, achieves the best results on these three benchmarks and has significant advantages on longer videos.}
    \label{fig1}
\end{figure}

Video-LMs typically encode a video as a sequence of visual tokens, which are then concatenated with language tokens into a long sequence and then use LLMs as decoders to understand this combined sequence. While Video-LMs improve video understanding, their performance is still limited. 
To handle longer videos, these methods typically perform uniform or random frame sampling at large strides without considering content~\cite{SeViLA}, leading to potential key information loss. Additionally, the simple concatenation of visual tokens increases the difficulty for the LLM to locate question-related (key) visual information within the long vision sequence, complicating long-range reasoning across the vision token sequences.

As discussed above, these two key issues in long video understanding remain challenging for current Video-LMs: accurately locating question-related video clips or images and reasoning over long sequences. While these problems are difficult for Video-LMs to solve, LLMs have demonstrated impressive capabilities in key information location and long-form reasoning on various language-only tasks, such as document retrieval and long-context understanding. Considering that some long videos, like movies, are initially written as scripts or books, humans can answer questions by either watching the videos or reading the books. Inspired by this observation, converting long-video understanding into a long-document understanding task may effectively leverage the power of large language models. Recent works~\cite{LLoVi} have attempted to develop strategies to convert videos into text captions and use LLMs for reasoning based on these captions. However, the challenge of converting a video into a long document without losing key information relevant to solving the question is not fully explored. Additionally, locating the key information (clips or frames) has not been thoroughly investigated.

 %DrVideo consists of %a Large Vision-Language Model (LVLM), a retrieval module, and a Large Language Model as the expert agent.
%five parts: Video-Document Conversion Module; Document Retrieval module; Document Augmentation Module; Multi-Stage Agent Interaction System, a Multi-Stage Agent Interaction Loop and an Answering Module

Therefore, in this paper, we propose DrVideo, a document retrieval-based system for long video understanding that progressively finds key frames and generates question-related information for LLMs to make confident predictions.
DrVideo comprises five components: (i) a video-document conversion module that transforms raw long videos into long documents, (ii) a retrieval module that identifies frames related to specific video questions, (iii) a document augmentation (DA) module that enriches the information of question-related frames (key frames), (iv) a multi-stage agent interaction loop that dynamically finds the potential missing information through sequential steps of reasoning and then interacts with the DA module to request augmentation of the information, (v) an answering module that provides answers and the logical process of obtaining those answers based on sufficient information.
We validate the effect of each component in Section \ref{experiment:ablation}. Extensive experiments show our method, DrVideo, exceeds existing state-of-the-art methods across different long video benchmarks, from 3 minutes to 10 minutes and longer than 1 hour, which are shown in Fig. \ref{fig1}.
Finally, we summarize the contributions of DrVideo in the following three aspects:
\begin{itemize}
\item A system is proposed to adapt long-video understanding to long-document understanding, which can better take advantage of the long-range reasoning ability of LLMs.
\item A novel multi-stage interactive loop is proposed to continuously search for missing information and dynamically augment the information.
\item DrVideo achieves state-of-the-art results on three long video benchmarks and exceeds existing state-of-the-art methods with +3.8 accuracy on the EgoSchema benchmark (3 minutes), +17.9 in MovieChat-1K breakpoint mode, +38.0 in MovieChat-1K global mode (10 minutes), and +30.2 on the LLama-Vid-QA dataset (over 60 minutes).
\end{itemize}%Short Long Video EgoSchema benchmark and middle lengthy video MovieChat-1K benchmark and achieves the best results on Ultra-long videos LLAMA-vid. 


%By conducting extensive experiments, we find DrVideo can generate better predictions than existing works. Moreover, DrVideo shows a large gap compared with previous work on the longest benchmark, MovieChat-1K, especially in its global mode which requires obtaining an answer by performing long-range reasoning across the entire long video. Finally, we summarize the contributions of DrVideo in the following three aspects.


%DrVideo begins by converting video frames into short descriptions using the LVLM, organizing these descriptions and corresponding frame IDs into an initial document. A retrieval augment (RA) module then identifies the top K question-related frames based on language similarity, and adopts LVLM to generates detailed captions for these key frames to provide more useful information. Using LLMs to directly generate predictions based on the current information can lead to suboptimal results due to missing frames or insufficient details. To address this, DrVideo incorporates a multi-stage interactive loop to find the missing key information. Specifically, this loop first uses the expert agent (e.g., GPT-4) to decide whether the current information is sufficient and accurate enough to answer the specific question. If the agent finds the information insufficient, it provides reasons and identifies the missing content, prompting the retrieval augment module to find more information based on these requests. Once enough information is collected to support a high-confidence prediction, the agent makes the final prediction in a chain-of-thought manner.





%Till this step, Given the video question and the short description of long video and detail description of retrived K frames, LLM can give the inital prediction.
% which can be considered as the agenda of the book.
%. A recent work ~\cite{LaViLa} adopts a simple framework, using a short-term visual captioner to generate captions for many clips at once and uses this as the document for LLM to analyze. However, this straightforward conversion strategy leads to missing information and introducing noise because the captioner is not question-aware.  Seconly





%Additionally, treating all frame captions as equally important introduces extra noise for LLMs
%, first one is the such caption is not question awared, it may generate the description doesn't realted to the question and would adding the noise the 




%capability for long-form reasoning on a wide range of tasks such as document retrieval and understanding 

%First one how to compress the number of tokens when encoding image or video clips.
%\textcolor{red}{need experiments}
%long-context understanding ability of Large Language Models (LLMs)\cite{brown2020language,chung2024scaling,touvron2023llama} , recent works attempts to use LLM to understand the longer video context. LLaMA-VID ~\cite{touvron2023llama}.
%\textcolor{red}{Need experiments to run Movidechat on LLAMA-vid}
%Understanding long-form videos, which can range from minutes to hours, requires a model that can process different types of information, handle very long sequences, and effectively analyze these sequences. Existing video-LM methods  \chenhui{We are not solving issues of Video-LM} have a maximum length limitation, making them unable to handle ultra-long sequences. Besides, long video sequences contain a large amount of irrelevant and redundant information, how to exactly find question relevant information and drop the noise and redundant information from long video sequences is a important challenge in the field of long-form video understanding.\par
%\\Recently, Large Language Models (LLMs) have shown impressive capability for long-form reasoning on a wide range of tasks such as document retrieval and understanding \cite{sun2023pearl}. Inspired by these results in the natural language and decision-making domain, we explore to translate the long video into long document and utilize the long context processing ability and the long-form temporal reasoning ability of LLMs for long form video understanding. Unlike prior long form video models, our approach does not require specialized long-form video modules (e.g., memory queues, state-space layers, spatio-temporal graphs, etc.) but instead uses \chenhui{ not short-term} a short-term visual captioner and an LLM to overcome the challenge of maximum length limitation. \chenhui{May be briefly talk this system first} Specially, given a long video input, we segment it into multiple short clips and convert them into one-sentence brief textual descriptions using a pre-trained frame/clip level visual captioner (e.g., LLaVA, LaViLa). In this situation, we can leverage the long context processing capabilities of LLM to handle these temporally ordered captions without worrying about the sequence length.\par

%\chenhui{put this one before explain how we convert} However, such vision-to-language conversion will lost much meaningful content which is crucial for accurately understanding the question related a long video. \chenhui{the next challenge of what, conversion or generation challenge } The next challenge is how to minimize the loss of key information related to the question while ensuring that the video length is not a limiting factor. To solve it, we introduce a retrieval model to identify the top question-related frames via calculate the similarity between the question and these temporally ordered captions. Afterward, a Large Multi-Modality Model (e.g., LLaVA-1.6) provides detailed descriptions of these identified frames to minimize the information loss. Our preliminary study finds that this retrieval-augmented \chenhui{where is augment} method can identify some key frames relevant to the question and reduce the loss of information in these key frames. However, the performance of this retrieval-augmented method is limited for two reasons: (i) this keyframe selection methods might select the wrong frames and mislead the model; (ii) apart from their own semantic information, more question related key frames need to be identified through contextual inference. Relying solely on semantic similarity calculations is insufficient for accurate determination.\par
%To find more question related key frames, we propose an agent-based loop up on the retrieval augmented module. This loop employs LLMs as agents, progressively refines the frame selection and interacts with the LMM to enhance descriptions and reduce the loss of key information. Specifically, this loop first use an LLM (e.g., GPT-4) to judge whether these augmented temporally ordered captions come from retrieval module are sufficient and accurate enough to answer the question related a long video. \chenhui{Too much detail} If the answer of the LLM is yes, it indicates that we do not need to find more question related key frames. If the answer of the LLM is no, it indicates that current augmented temporally ordered captions come from retrieval module are insufficient to answer the question accurately. Then another LLM along with a LMM \chenhui{Too much LLM,LMM, get confusing} is used to find more question related key frames and enhance these frames with more detailed descriptions. Finally, the updated augmented temporally ordered captions once again feed into the first LLM to judge whether the updated captions are sufficient to answer the question. Our agent-based loop progressively refines the frame selection and enhance these descriptions to minimize the loss of key information.\par
%After obtained those updated augmented temporally ordered captions, the next challenge is how to correctly predict the answer from these captions, which contain a large amount of information and the length of all captions is very long. Inspired by the long-form temporal reasoning ability of LLM, we feed these captions to the LLM with chain of thought prompt to reason the correct answer.\par
%To bridge the above-mentioned research gaps, we propose DrLongVideo, a retrieval-augmented agent-based system for long video understanding. This system contains three parts: (i) the first part is to translate the raw long video sequence into a long document using a pre-trained frame/clip level visual captioner, and then introduce a retrieval model to identify the initial question-related frames via calculate the similarity between the question and these temporally ordered captions. (ii) the second part is an agent-based loop up on the retrieval module to judge the augmented caption whether satisfied with answer the question and find more question related key frames via LLM interacts with LMM. (iii) the last part is to reason these captions with chain of thought prompt to predict final answer.\par
%Our work differs from previous works in two aspects: Compared to the works that 
%require costly and complex specialized long-form video modules (e.g., memory queues, state-space layers, spatio-temporal graphs, etc.), our method is more simple and more effective under training-free setting in long video which ranges from minutes to hours. Compared to the works that uniformly sample frames or select frames in a single iteration, our method selects frames via a retrieval model and an agent-based loop to find the question related frames and enhance these frames with detailed descriptions in a multi-round fashion, which ensure the information gathered to be more accurate based on the current need.\par
%Our rigorous evaluation of two well-established long-form video understanding benchmarks, EgoSchema and MovieChat-1K, demonstrates DrLongVideo's exceptional effectiveness compared to existing methods. DrLongVideo achieves 61\% and xx\% accuracy on these two benchmarks, respectively, outperforming concurrent state-of-the-art method LLoVi by 10.3\% on EgoSchema benchmark and the state-of-the-art method MovieChat by xx\% on MovieChat-1K benchmark. Our ablation studies highlight the significance of the document retrieve augmented and the key frame selection progressively in a iterative process, which adaptively searches and aggregates relevant information based on the complexity of the videos. Furthermore, we extend our DrLongVideo to the hour-level long video benchmark LLaMA-VID, indicating that DrLongVideo outperforms existing state-of-the-art methods by a margin.\par
%To summarize, this work has the following contributions:\par
%1) We propose DrLongVideo, a retrieval-augmented agent-based system for long video understanding. Different the works that uniformly sample frames or select frames in a single iteration, our method selects frames via a retrieval model and an agent-based loop to find the question related frames and enhance these frames with detailed descriptions in a multi-round fashion. This is first study to explore the effectiveness of document retrieval and LLM-agent in long form video understanding task.\par
%2) DrLongVideo outperforms all existing state-of-the-art methods on EgoSchema subset and fullset, MovieChat-1K, and LLaMA-VID benchmarks, with testing accuracies of 61\%, xx\%, and xx\%, respectively. \chenhui{double check this one, whether we can see outperforms all}



==> sec/sections/methods_abortion.tex <==
\begin{algorithm}[htbp]
\caption{DrVideo}
\label{alg:drvideo}
\begin{algorithmic}[1]
\Require $V$, $Q$%, LLM $\phi_{llm}$, VLM $\phi_{vlm}$, 
max iteration $I$
\State \textbf{$\blacktriangleright$ Video-Document Conversion}
\State \hspace{1em}$init$ \space $\phi_{emb}$, $\phi_{vlm}, \mathcal{P}$
\State \hspace{1em}$\mathcal{E}_{\text{doc}} \gets \phi_{emb}(\text{Doc})$; $\text{Doc} \gets \left\{...,\{T, S_{V_T}\} \right\}$; $S_{V_t} \gets \phi_{vlm}(\mathcal{P}, V_t)$
\State \textbf{$\blacktriangleright$ Retrieval Augmentation Module}
 \State \hspace{1em} $init$ $\mathcal{RT}$, $\mathcal{AP}$, $\phi_{emb}$, $K$
 \State \hspace{1em}  $\text{topk\_doc} \gets Retrieval(\mathcal{RT},$\text{Doc}$,K) $
 \State \hspace{1em}  $\mathcal{AD}_0 \gets Augment(\text{topk\_doc},\text{Doc},\mathcal{AP})$
%\State  \hspace{1em}$\mathcal{E}_{\mathcal{RT}} \gets \phi_{emb}(\mathcal{RT})$; $\phi_{emb}(\mathcal{RT})$;
%\State \hspace{1em} $\text{topk\_doc} \gets \text{arg\,topK}_t (\mathcal{E}_{\mathcal{RT}}, \mathcal{E}_{\text{doc}_t})$
%\State \hspace{1em} \textbf{for} each $t' \in \text{topk\_doc}$: $L_{V_{t'}} \gets \phi_{vlm}(\mathcal{P}, \mathcal{AP})$
%\State \hspace{1em}  $\mathcal{AD}_0 \gets \text{Get_augmented Doc}$%\left\{ 
%\begin{cases} 
%\{t, S_{V_t}, L_{V_t'}\} & \text{if } t = t' \\
%\{t, S_{V_t}\} & \text{otherwise}
%\end{cases} \mid t = 1, 2, \ldots, T \right\}$
\State \textbf{$\blacktriangleright$ Multi-Stage Agent Interaction}
\State \hspace{1em}$init$ i=0
%\setlength{\algorithmicindent}{1em} 
%\While{not final}
\State \hspace{1em} \textbf{For} $i \leq I$:%not final
    \State \hspace{2em}\textbf{Planning Agent:}
    \State \hspace{3em} sufficient = Sufficient($\mathcal{AD}_i$)
    %\If{sufficient}
    \State \hspace{3em} \textbf{If} sufficient  
     \State \hspace{4em} \textbf{then}  
     \State \hspace{5em}  break
    %\Else
    \State \hspace{4em} \textbf{else} 
        \State \hspace{5em} call Interaction Agent
    \State \hspace{2em}\textbf{Interaction Agent:}
    \State \hspace{3em} f%Analyze $\mathcal{AD}_i$ and reasons, identify missing information
    \State \hspace{3em} Update retrieval text $\mathcal{RT}_i$ and decide on best Augment Prompt $\mathcal{AP}_i$

    \State \hspace{2em} \textbf{Interaction with RA:}
    \State \hspace{3em} Getting AD \text{topk\_doc} ensuring: $\text{topk\_doc} = \text{arg\,topK}_t (\mathcal{E}_{\mathcal{RT}}$, $\forall n \in M, \quad n \in T, \quad n \notin \text{topk\_doc}$,
    %\[
    %\forall n \in M, \quad n \in T, \quad n \notin \text{topk\_doc}, \quad \text{and} \quad N < K
    %\]
    \State Use $\mathcal{AP}_i$ to query VLM for detailed information
%\EndWhile

\State \textbf{Answering Module:}
\State Generate final prediction based on collected information
\Return $\hat{Y}$

\end{algorithmic}
\end{algorithm}

\begin{algorithm}[htbp]
\caption{DrVideo}
\label{alg:drvideo}
\begin{algorithmic}[1]
\Require $V, Q,\phi_{vlm},\phi_{emb},\phi_{LLM}, I, K$
\State \textbf{$\blacktriangleright$ Video-Document Conversion}
\State \hspace{1em}$init$\space  $\mathcal{P}$
\State \hspace{1em}$\text{Doc} \gets getDoc(V,\phi_{vlm},\mathcal{P}$);
\State \hspace{1em}$\mathcal{E\_{\text{doc}}} \gets getEmedding(\text{Doc} ,\phi_{emb}$);
%\State \hspace{1em}$\mathcal{E}_{\text{doc}} \gets \phi_{emb}(\text{Doc})$; $\text{Doc} \gets \left\{...,\{T, S_{V_T}\} \right\}$; $S_{V_t} \gets \phi_{vlm}(\mathcal{P}, V_t)$
\State \textbf{$\blacktriangleright$ Retrieval Augmentation Module}
 \State \hspace{1em} $init$ $\mathcal{RT}$, $\mathcal{AP}$,
 \State \hspace{1em} $ \mathcal{E}_{\mathcal{RT}} \gets getEmedding(\mathcal{RT} ,\phi_{emb}$);
 \State \hspace{1em}  $\text{topk\_doc} \gets Retrieval(\mathcal{E}_{\mathcal{RT}},\text{Doc},K) $
 
 \State \hspace{1em}  $\mathcal{AD}_0 \gets Augment(\text{topk\_doc},\text{Doc},\mathcal{AP})$
\State \textbf{$\blacktriangleright$ Multi-Stage Agent Interaction}
\State \hspace{1em}$init$ i=0
%\setlength{\algorithmicindent}{1em} 
%\While{not final}
\State \hspace{1em} \textbf{For} $i \leq I$:%not final
    \State \hspace{2em}\textbf{Planning Agent:}
    \State \hspace{3em} $\mathcal{S} = CheckSufficient(\mathcal{AD}_i$)
    %\If{sufficient}
    \State \hspace{3em} \textbf{If} S  
     \State \hspace{4em} \textbf{then}
     \State \hspace{5em}  break
    %\Else
    \State \hspace{4em} \textbf{else} 
    \State \hspace{5em} $\mathcal{R}_i= Analyze(\mathcal{AD}_i)$
    \State \hspace{2em}\textbf{Interaction Agent:}
    %\State \hspace{3em} %Analyze $\mathcal{AD}_i$ and reasons, identify missing information
    \State \hspace{3em} $$ \gets $FindMissInfo(\mathcal{AD}_i,\mathcal{R}_i)$
    \State \hspace{2em} \textbf{Interaction with RA:}
    \State \hspace{3em} $\text{topn\_doc} \gets \text{arg\,topK}_t (\mathcal{E}_{\mathcal{RT}}$, $\forall n \in M, \quad n \in T, \quad n \notin \text{topk\_doc}$,
    %\[
    %\forall n \in M, \quad n \in T, \quad n \notin \text{topk\_doc}, \quad \text{and} \quad N < K
    %\]
    \State Use $\mathcal{AP}_i$ to query VLM for detailed information
%\EndWhile

\State \textbf{Answering Module:}
\State Generate final prediction based on collected information
\Return $\hat{Y}$

\end{algorithmic}
\end{algorithm}

==> sec/sections/related_work.tex <==
\section{Related Work}
\noindent \textbf{Long Video Understanding.} Modeling long videos, which are several minutes or more in length, generally necessitates advanced temporal modeling capabilities, resulting in complex model designs. LF-VILA~\cite{sun2022long} introduces a Temporal Window Attention (HTWA) mechanism to capture long-range dependencies in long videos. MeMViT~\cite{wu2022memvit} and MovieChat~\cite{song2023moviechat} employs a memory-based design to save question-related information from previously video segments. Some published approaches employ space-time graphs~\cite{hussein2019videograph,wang2021supervoxel} or relational space-time modules~\cite{yang2023relational} to capture spatio-temporal dependencies from the raw long videos. Recently, S4ND~\cite{nguyen2022s4nd}, ViS4mer~\cite{islam2022long}, and S5~\cite{wang2023selective} have used Structured State-Space Sequence (S4)~\cite{gu2021efficiently} layers to capture long-range dependencies in videos. Different from these methods, our DrVideo does not design a complex module to perform long video understanding capacity. On the contrary, we develop a document-retrieval-based system for zero-shot long video understanding.
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.63]{./image/drvideo_2.pdf}

    \caption{\textbf{Overview of our DrVideo.} It comprises five components: a video-document conversion module, a retrieval module, a document augmentation module, a multi-stage agent interaction loop and an answering module.}
    \label{fig2}
\end{figure*}



\noindent \textbf{LLMs for Video Understanding.} 
The recent rise of LLMs \cite{zeng2022socraticmodels} and VideoChat~\cite{li2023videochat} align the visual features extracted by pretrained visual models to LLMs and apply them into video understanding filed. Video ChatCaptioner~\cite{chen2023video} and ChatVideo~\cite{wang2023chatvideo} utilize LLMs to represent videos and engage users through dialogues, respectively. VidIL~\cite{wang2022language} applies the image-level models into video understanding task via few-shot learning. In addition to short-term video understanding, recent studies~\cite{2023mmvid,chung2023long,bhattacharya2023video} have explored LLMs for long-range video modeling. For instance, GPT-4 is applied in various long-range video modeling tasks in~\cite{2023mmvid}, though quantitative evaluation is limited. Meanwhile, research in~\cite{chung2023long} focuses on movie datasets with minimal visual analysis~\cite{mangalam2023egoschema}, relying largely on speech and subtitles. Unlike this, DrVideo focuses on vision modality and never uses the prior language information.
%NextQA~\cite{xiao2021next}, 

\noindent \textbf{LLM Agents.} 
In parallel, the computer vision community has started exploring the use of LLMs as agents in various visual domains like GUI understanding and robot navigation~\cite{suris2023vipergpt,hong2023cogagent,driess2023palm,brohan2023rt}. In the realm of long-form video comprehension, initial efforts have employed an agent-like approach, where LLMs interact with external tools or integrate additional functionalities~\cite{suris2023vipergpt,gao2023assistgpt,yang2024doraemongpt,wang2024videoagent,fan2024videoagent}. In contrast to these approaches, our method, DrVideo, reconceptualizes video understanding as a process augmented by document retrieval, inspired by how humans watch videos or read books. This view leads to the development of DrVideo, which features document retrieval augmentation and multi-stage interactivity to distinguish it from existing methods.


